Total Stability of SVMs and Localized SVMs

Regularized kernel-based methods such as support vector machines (SVMs) typically depend on the underlying probability measure $\mathrm{P}$ (respectively an empirical measure $\mathrm{D}_n$ in applications) as well as on the regularization parameter $\lambda$ and the kernel $k$. Whereas classical statistical robustness only considers the effect of small perturbations in $\mathrm{P}$, the present paper investigates the influence of simultaneous slight variations in the whole triple $(\mathrm{P},\lambda,k)$, respectively $(\mathrm{D}_n,\lambda_n,k)$, on the resulting predictor. Existing results from the literature are considerably generalized and improved. In order to also make them applicable to big data, where regular SVMs suffer from their super-linear computational requirements, we show how our results can be transferred to the context of localized learning. Here, the effect of slight variations in the applied regionalization, which might for example stem from changes in $\mathrm{P}$ respectively $\mathrm{D}_n$, is considered as well.

==> Sections/04_Loc_GleicheAufteilung.tex <==
\subsection{Same regionalization for both localized SVMs}\label{SubSec:Rob_Loc_SameLoc}

First, we assume that both of the global predictors we want to compare in order to assess the stability of this localized approach are based on the same regionalization. Our stability result will not be based on any specific regionalization method but rather can be applied to any regionalization satisfying some very mild conditions. We will denote this regionalization by $\XBbold := \{\X_1,\dots,\X_B\}$ for some sets $\X_1,\dots,\X_B$ such that the following holds true:

\begin{description}
	\item[(R1)] $\X_1,\dots,\X_B \subseteq \X$ and $\X=\bigcup_{b=1}^B \X_b$. \red{Wäre eigentlich nicht nötig für Resultate}
\end{description}
Additionally, \XBbold needs to satisfy the following condition for whichever probability measure \P our localized SVM is based on:
\begin{description}
	\item[(R2)] $\P(\X_b\times\Y) > 0$ for all $b\in\{1,\dots,B\}$.
\end{description}
Note that \textbf{(R1)} tells us that the regions need not necessarily be pairwise disjoint but can instead also overlap. Condition \textbf{(R2)} of no region having probability mass zero is trivially needed since the local SVM on the respective region would not be defined elsewise.

Since we want to investigate stability similarly to \Cref{Thm:Rob_Stability}, we again assume to have two possibly different Borel probability measures $\P_1$ and $\P_2$ on \XY which the predictors we want to compare are based on. For obtaining local SVMs on $\X_1,\dots,\X_B$ for our localized approach, we now first need to introduce the associated local probability measures on these regions (respectively on $\Xb\times\Y$, $b=1,\dots,B$) by restricting $\P_1$ and $\P_2$: On an arbitrary $\tilde{\X}\subseteq\X$ satisfying $\P_i(\tilde{\X}\times\Y)>0$, we define the local probability measure based on $\P_i$ by
\begin{align}\label{eq:Rob_Loc_Pib}
	\P_{i,\tilde{\X}} := \frac{1}{\P_i(\tilde{\X}\times\Y)}\cdot (\P_i)\einschraenkung_{\tilde{\X}\times\Y}\,,\qquad i\in\{1,2\}.
\end{align}
If the regionalization satisfies \textbf{(R2)} for $\P_1$ and $\P_2$, these local probability measures are obviously well-defined on any $\Xb$, $b\in\{1,\dots,B\}$. Since we will mainly need the local probability measures on these sets from \XBbold, we also write $\Pib:=\P_{i,\Xb}$ to shorten the notation, $i=1,2$, $b=1,\dots,B$.

As mentioned in \Cref{Sec:Rob_Intro}, one big advantage of such localized approaches lies in their increased flexibility with regards to learning a function whose complexity and volatility vary across the input space since areas with differing complexities of the function can be separated into different regions. Hence, it should obviously be possible to choose different regularization parameters and kernels in the different regions because they to some extent control the complexity of the resulting SVM. We therefore have vectors of regularization parameters $\lbibold := (\lb_{i,1},\dots,\lb_{i,B})$, with $\lb_{i,b}>0$ for all $b\in\{1,\dots,B\}$, and vectors of kernels $\kibold := (\k_{i,1},\dots,\k_{i,B})$, for $i=1,2$. Based on these and a shifted loss function \lossshift, we obtain from \eqref{eq:Rob_DefShiftSVM} SVMs 
\begin{align*}
	\fibext : \Xb\to\R\,, \qquad i\in\{1,2\},\, b\in\{1,\dots,B\}
\end{align*}
which we call \it local SVMs \rm on \Xb.

For combining these local SVMs and thus obtaining a global predictor on \X, we first need to extend them in a way such that they are defined on all of \X. That is, for a function $g:\tilde{\X}\to\R$ on $\tilde{\X}\subseteq\X$, we define the zero-extension $\hat{g}:\X\to\R$ by
\begin{align*}
	\hat{g}(x) := \begin{cases}
		g(x) &\wenn x\in\tilde{\X}\,,\\
		0 &\sonst\,.
	\end{cases}
\end{align*}
Later on we will also need zero-extensions of kernels and probability measures which we also indicate by using the $(\hat{\cdot})$-notation: If $\k:\tilde{\X}\times\tilde{\X}\to\R$ is a kernel on $\tilde{\X}\subseteq\X$, we define $\hat{\k}:\XX\to\R$ by
\begin{align*}
	\hat{\k}(x_1,x_2) := \begin{cases}
		k(x_1,x_2) &\wenn x_1,x_2\in\tilde{\X}\,,\\
		0 &\sonst\,.
	\end{cases}
\end{align*}
If \Q is a Borel probability measure on $\tilde{\X}\times\Y$ with $\tilde{\X}\subseteq\X$, we define $\hat{\Q}:\BXY\to[0,1]$ by
\begin{align*}
	\hat{\Q}(A) := \Q\left(A\cap\left(\tilde{\X}\times\Y\right)\right)\,.
\end{align*}
Here, \BXY denotes the Borel $\sigma$-algebra on \XY.

Before finally defining our global predictors, we lastly also need weight functions $w_b$, $b\in\{1,\dots,B\}$, which pointwisely control the influence of the different local SVMs in areas where two or more regions overlap. These weight functions are required to satisfy the following three conditions: 
\begin{description}
	\item[(W1)] $w_b:\X\to[0,1]$ for all $b\in\{1,\dots,B\}$.
	\item[(W2)] $\sum_{b=1}^B w_b(x) = 1$ for all $x\in\X$.
	\item[(W3)] $w_b(x)=0$ for all $x\notin\Xb$ and all $b\in\{1,\dots,B\}$.
\end{description}
\red{Exakt wie in \cite{dumpert2018}; (W3) wird eigentlich nicht benötigt, da Funktionen dort eh 0 sind}

With this, we define global predictors \fiext[1] and \fiext[2], which we will call \it localized SVMs \rm even though they are not necessarily SVMs themselves, by
\begin{align}\label{eq:Rob_Loc_DefGlobalPredictor}
	\fiext: \X\to\R\,,\, x\mapsto \sum_{b=1}^{B} w_b(x) \cdot \fibextdach(x)
\end{align}
for $i=1,2$, where we again omitted the shifted loss function \lossshift to shorten the notation.

The succeeding theorem states that \Cref{Thm:Rob_Stability} can be transferred to the situation at hand, \ie that such localized SVMs inherit a similar stability property from regular SVMs:

\begin{mythm}\label{Thm:Rob_Loc_GleicheAufteilung}
	Let \X be a complete and separable metric space and $\Y\subseteq\R$ be closed. Let $\P_1,\P_2\in\MXY$ be probability measures. Let $\XBbold:=\{\X_1,\dots,\X_B\}$ be a regionalization of \X such that \XBbold satisfies \textbf{(R1)} and, for $\P_1$ as well as for $\P_2$, \textbf{(R2)}. Let $\lbib>0$ and let $\kib$ be a bounded and measurable kernel with separable RKHS $\Hib$ for all $i\in\{1,2\}$ and $b\in\{1,\dots,B\}$. Denote $\kappa_b:=\max\{\normSup{\kib[1]},\normSup{\kib[2]}\}$ and $\tau_b:=\min\{\lbib[1],\lbib[2]\}$ for all $b\in\{1,\dots,B\}$. Let \loss be a convex and Lipschitz continuous loss function. Let \fiext[1] and \fiext[2] be defined as in \eqref{eq:Rob_Loc_DefGlobalPredictor} with the weight functions $w_1,\dots,w_B$ satisfying \textbf{(W1)}, \textbf{(W2)} and \textbf{(W3)}. Then,
	\begin{align*}
		\normSup{\fiext[1]-\fiext[2]} \le |\loss|_1 \cdot \max_{b\in\{1,\dots,B\}} \frac{1}{\tau_b} \cdot  &\left( \kappa_b^2\cdot \norm{tv}{\Pib[1]-\Pib[2]} + \frac{\kappa_b^2}{\tau_b}\cdot |\lbib[1]-\lbib[2]|\right.\\ 
		&\hspace*{1cm}+ \frac{1}{2} \cdot \normSup{\kib[1]-\kib[2]}\\ 
		&\hspace*{2cm}+ \kappa_b \cdot \sqrt{\normSup{\kib[1]-\kib[2]}} \bigg)\,.
	\end{align*}
	%as well as, for all probability measures $\Q\in\MX$ on \X and for all $p\in[1,\infty)$,
	%\begin{align*}
	%	&\norm{\Lp(\Q)}{\fiext[1]-\fiext[2]}\\ 
	%	&\le |\loss|_1 \cdot \left(\sum_{b=1}^B \Q(\Xb) \cdot \right.\left( \frac{\kappa_b^2}{\tau_b}\cdot \norm{tv}{\Pib[1]-\Pib[2]} + \frac{\kappa_b^2}{\tau_b^2}\cdot |\lbib[1]-\lbib[2]|\right.\\
	%	&\hspace*{5cm}\left.+ \frac{1}{2\tau_b} \cdot \normSup{\kib[1]-\kib[2]} + \frac{\kappa_b}{\tau_b} \cdot \sqrt{\normSup{\kib[1]-\kib[2]}} \right)^p\Bigg)^{1/p}\,.
	%\end{align*}
\end{mythm}

Similarly, we can also transfer \Cref{Thm:Rob_StabilityLp} in order to bound the \Lppix-norm of the difference:

\begin{mythm}
	\label{Thm:Rob_Loc_GleicheAufteilungLp}
	Let \X be a complete and separable metric space and $\Y\subseteq\R$ be closed. Let $\P_1,\P_2\in\MXY$ be probability measures. Let $\XBbold:=\{\X_1,\dots,\X_B\}$ be a regionalization of \X such that \XBbold satisfies \textbf{(R1)} and, for $\P_1$ as well as for $\P_2$, \textbf{(R2)}. Let $\lbib>0$ and let $\kib$ be a bounded and measurable kernel with separable RKHS $\Hib$ for all $i\in\{1,2\}$ and $b\in\{1,\dots,B\}$. Denote $\kappa_b:=\max\{\normSup{\kib[1]},\normSup{\kib[2]}\}$ and $\tau_b:=\min\{\lbib[1],\lbib[2]\}$ for all $b\in\{1,\dots,B\}$. Let \loss be a convex and Lipschitz continuous loss function. Let \fiext[1] and \fiext[2] be defined as in \eqref{eq:Rob_Loc_DefGlobalPredictor} with the weight functions $w_1,\dots,w_B$ satisfying \textbf{(W1)}, \textbf{(W2)} and \textbf{(W3)} \red{Eigentlich nur (W1) nötig}. Then, for all $p\in[1,\infty)$ and all $i\in\{1,2\}$,
	\begin{align*}
		&\normLppix{\fiext[1]-\fiext[2]}\\ 
		&\le |\loss|_1 \cdot \sum_{b=1}^B \left(\Pix(\Xb)\right)^{1/p} \cdot  \left( \frac{\kappa_b^2}{\tau_b}\cdot \norm{tv}{\Pib[1]-\Pib[2]} + \frac{\kappa_b^2}{\tau_b^2}\cdot |\lbib[1]-\lbib[2]|\right.\\
		&\hspace*{6cm}+ \frac{1}{2\tau_b} \cdot \normLppibxb{\kib[1]-\kib[2]}\\
		&\hspace*{7cm}\left.+ \frac{\kappa_b}{\tau_b} \cdot \sqrt{\normLppibxb{\kib[1]-\kib[2]}} \right)\,.
	\end{align*}
\end{mythm}


==> Sections/05_Loc_VerschAuft.tex <==
\subsection{Different regionalizations for the localized SVMs}\label{SubSec:Rob_Loc_DiffLoc}


In the previous section, we investigated stability of localized SVMs with respect to changes in the triple $(\P,\lbbold,\kbold)$ but not in the regionalization. However, when there are changes in the distribution \P used for calculating the localized SVM (\eg because of changes in the training data set in practice), it may very well happen that this also affects the regionalization if it is not predetermined but also based on a learning method (for example decision respectively regression trees, \vgl \cite{chang2010} among others \red{In Einleitung mehr genannt}). Hence, we will now take a closer look at the effect of slight changes in the regionalization (in addition to those in $(\P,\lbbold,\kbold)$) on the resulting localized SVM in this section. 

First of all, it has to be mentioned that we will sadly not be able to derive a meaningful result regarding the uniform norm of the difference of two such localized SVMs (like \Cref{Thm:Rob_Loc_GleicheAufteilung} in the case of coinciding regionalizations), which can readily be seen from the simple example visualized in \Cref{Abb:Rob_Loc_DiffRegion}. There, two localized SVMs are being compared. Both of them are based on the same training data (\ie on the same distribution) generated according to
\begin{align*}
	X \sim \unif[-1,1]\,,\qquad Y|X \sim \text{sign}(X) + \eps \text{ with } \eps \sim \normal[0,0.01]\,.
\end{align*} 
\red{(Notation erklären)} Furthermore, both localized SVMs use the same regularization parameters and the same kernel on every region. They only differ in the underlying regionalization: The input space in split into two parts in both bases, but for \fa the border between the two regions is at $x=0$ (thus exactly capturing the pattern in the data) whereas it is moved slightly to the right, to $x=0.035$, for \fb. 
%On a side note, it is of course also possible for regular SVMs to approximate underlying functions with such discontinuities well, given enough training data. This follows from their universal consistency, \vgl Theorem 9 from \cite{christmann2009}. In the special case of this example however, the left part of \fb is not able to capture the discontinuity at all since it incorporates too few data on the right hand side of it and these are greatly outweighed by the rest of the data, in addition to using rather strong regularization.

\begin{figure}
	\begin{center}
		\vspace*{-0.5cm}\includegraphics[width=0.7\textwidth]{PlotLocalizedSVMs}
		\vspace*{-0.5cm}\caption{Comparison of two localized SVMs based on the same distribution, regularization parameters and kernels but on different regionalizations.}
		\label{Abb:Rob_Loc_DiffRegion}
	\end{center}
\end{figure}

Though it can easily be seen from \Cref{Abb:Rob_Loc_DiffRegion} that this very minor change in the regionalization greatly impacts the maximum difference between \fa and \fb and it is obviously not possible to bound this maximum difference between two localized SVMs in any meaningful way, the same \Cref{Abb:Rob_Loc_DiffRegion} also suggests that it might still be possible to find such meaningful bounds on the \Lapix-norm of the difference (which is rather small in the example, less than $0.03$, compared to the uniform norm of approximately $1.3$), similarly to \Cref{Thm:Rob_Loc_GleicheAufteilungLp} and again based on \Cref{Thm:Rob_StabilityLp}. This will indeed be the case, but before stating the corresponding theorem, we first need to modify some of the notation introduced in \Cref{SubSec:Rob_Loc_SameLoc} such that it fits this new situation:

First of all, we now have two different regionalizations $\XiAibold[1] := \{\Xiaflex{1}{1},\dots,\Xiaflex{1}{A_1}\}$ and $\XiAibold[2] := \{\Xiaflex{2}{1},\dots,\Xiaflex{2}{A_2}\}$. Contrary to \Cref{SubSec:Rob_Loc_SameLoc}, we now require these regionalizations to actually be partitions of \X, \ie to satisfy the following modified version of \textbf{(R1)}:
\begin{description}
	\item[(R1')] $\Xiaflex{i}{1},\dots,\Xiaflex{i}{A_i}\subseteq\X$ and $\X=\bigcupdot_{a=1}^{A_i} \Xia$. \red{Erklären, was Punkt in Vereinigung bedeutet?}
\end{description}
Furthermore, we also need to alter \textbf{(R2)} slightly since our proofs in this section will use auxiliary SVMs defined on all possible intersections of sets from \XiAibold[1] with sets from \XiAibold[2], which is why all these intersections need to have positive probability with respect to the probability measure \P our localized SVM will be based on:
\begin{description}[labelwidth=\widthof{\bfseries (R2')},leftmargin=!]
	\item[(R2')] $\P(\Xbstar\times\Y)>0$ for all $\Xbstar \in \XBstarbold := \{\Xbstar[1],\dots,\Xbstar[B]\} := \{\X^*\subseteq\X \,|\, \exists \Xiai[1]\in\XiAibold[1],\Xiai[2]\in\XiAibold[2] : \X^* = \Xiai[1] \cap \Xiai[2] \} \setminus \{\emptyset\}$. We denote $J_{i,a}:=\{b\in\{1,\dots,B\}\,\left|\,\Xbstar\subseteq\Xia\right.\}\ne\emptyset$ for $i=1,2$ and $a=1,\dots,A_i$.
\end{description}

We can define local probability measures as before, \vgl \eqref{eq:Rob_Loc_Pib}, and will again shorten the notation for the ones we will mainly use: $\Pia:=\P_{i,\Xia}$, $i=1,2$, $a=1,\dots,A_i$. We then obtain local SVMs
\begin{align*}
	\fiaext : \Xia\to\R,\qquad i\in\{1,2\},\, a\in\{1,\dots,A_i\}
\end{align*}
based on regularization parameters $\lbia>0$ and kernels $\kia$. 

For combining these local SVMs in order to obtain our global predictors, no weight functions are needed this time, since the regions from the regionalizations are not allowed to overlap, \vgl \textbf{(R1')}. Thus, our localized SVMs are now readily defined as 
\begin{align}\label{eq:Rob_Loc_DefGlobalPredictorDiffLoc}
	\fiextreg: \X\to\R\,,\, x\mapsto \sum_{a=1}^{A_i} \fiaextdach(x)
\end{align}
for $i=1,2$, where $\lbibold:=(\lb_{i,1},\dots,\lb_{i,A_i})$ and $\kibold:=(\k_{i,1},\dots,\k_{i,A_i})$, again omitting the shifted loss function \lossshift to shorten the notation.

As before, we will investigate stability by bounding some norm of the difference of two estimators, in this case of two localized SVMs, based on how much the underlying probability measures and the vectors of regularization parameters and kernels differ. Now, the regionalizations are now added as a fourth possible difference. In order to base on our new bound on the difference between the two underlying regionalizations, we first have to somehow quantify this difference. We will base this quantification on the intersections between regions from the different regionalizations, \ie on the sets $\Xbstar[1],\dots,\Xbstar[B]$ from \textbf{(R2')}. For each of these intersections, we look at two properties which both in some sense characterize the difference between the two regionalizations: Firstly, it has to be considered how much the two intersecting regions producing \Xbstar differ in size -- relatively to these regions' own size and with respect to some probability measure \Q on \X. That is, we have to include the term
\begin{align}\label{eq:Rob_Loc_Versch_DiffRegPartI}
	\frac{\left|\Q(\Xiaib[1])-\Q(\Xiaib[2])\right|}{\max\left\{\Q(\Xiaib[1]),\Q(\Xiaib[2])\right\}}
\end{align}
for each such intersection, \ie for each $b\in\{1,\dots,B\}$. That is, a large difference in size could possibly lead to the local SVM on the smaller of the two regions being fitted much closer to its underlying data \red{(Genauer! Oder komplett weglassen)} and the two local SVMs therefore greatly differing on the regions' intersection \Xbstar. Secondly, we also have to consider how closely each region from \XiAibold[1] as well as from \XiAibold[2] coincides with one of the intersections $\Xbstar[1],\dots,\Xbstar[B]$, \ie how well each such region can be identified with a region from the other regionalization, again with respect to some probability measure \Q on \X. In order to control this property, we will include the term
\begin{align}\label{eq:Rob_Loc_Versch_DiffRegPartII}
	\Q_{\Xiaib}(\Xbstar)\cdot \left(1-\Q_{\Xiaib}(\Xbstar)\right)
\end{align}
for each $b\in\{1,\dots,B\}$ and $i\in\{1,2\}$. If a region \Xia closely coincides with \Xbstar for some $b\in J_{i,a}$, then $\Q_{\Xia}(\Xbstar)$ will be either close to 1 or close to 0, and \eqref{eq:Rob_Loc_Versch_DiffRegPartII} will hence be small, for each $b\in J_{i,a}$. If this is the case for all $i\in\{1,2\}$ and $a\in\{1,\dots,A_i\}$, each region can be identified well with a region from the other regionalization and the two regionalizations are therefore similar to each other in the sense of this second criterion. \red{(Evtl noch erklären weshalb dieses Kriterium wichtig ist)} 

\begin{figure}
	\begin{center}
		\vspace*{-1cm}\includegraphics[width=0.8\textwidth]{SimilarityRegionalizations}
		\vspace*{-1cm}\caption{Examples of intersections (red) of regions, for which (i) both; (ii) both; (iii) the second but not the first; (iv) the first but not the second; (v) neither the first nor the second; of the two difference criteria influencing \eqref{eq:Rob_Loc_Versch_DiffRegGesamt} is/are close to 0. \red{Nummern in Graphik aufnehmen.}}
		\label{Abb:Rob_Loc_SimilarityRegionalizations}
	\end{center}
\end{figure}

In \Cref{Abb:Rob_Loc_SimilarityRegionalizations}, we can see examples of intersections satisfying respectively not satisfying the two criteria we introduced (\ie, the respective terms being close to 0 respectively not close to 0). Here we assume the probability measure \Q used to investigate the difference to be that of a uniform distribution such that the intervals' sizes with respect to \Q coincide with their lengths. (i) and (ii) show the two types of intersections we assume to find if the regionalizations are similar to each other: Regions from the two regionalizations either almost coincide ((ii)) or overlap only slightly ((i)). It is easy to see that both criteria are satisfied in these cases. In (iii), the second criterion is still satisfied, \ie the intersection is either only a small part or almost the whole region for both regions assigned to it. However, the two regions greatly differ in size which increases \eqref{eq:Rob_Loc_Versch_DiffRegPartI} and makes the regionalizations more dissimilar. On the other hand, in (iv), the two intersecting regions are equal in size but their intersection coincides with exactly half of each of the two regions, resulting in both of them not being clearly assigned to one intersection and in increased values for the term from \eqref{eq:Rob_Loc_Versch_DiffRegPartII}. Lastly, (v) shows an example of an intersection for which none of the two criteria are satisfied (\eqref{eq:Rob_Loc_Versch_DiffRegPartII} indeed takes a small value for the second of the two intersecting regions, but not for the first one).

We now combine these two criteria in order to obtain a quantity to measure the difference between \XiAibold[1] and \XiAibold[2]. Since we analyzed the two criteria intersection-wise, we also define the quantification of this difference intersection-wise, \ie
\begin{align}\label{eq:Rob_Loc_Versch_DiffRegGesamt}
	\distReg{\Q}(\XiAibold[1],\XiAibold[2]) :=&\ \frac{\left|\Q(\Xiaib[1])-\Q(\Xiaib[2])\right|}{\max\left\{\Q(\Xiaib[1]),\Q(\Xiaib[2])\right\}}\notag\\ 
	&\ + \sum_{i=1}^{2} \bigg(\frac{1}{2}\cdot\Q_{\Xiaib}(\Xbstar)\cdot \left(1-\Q_{\Xiaib}(\Xbstar)\right)\notag\\ 
	&\ \hspace*{2cm} \left.+ \sqrt{\Q_{\Xiaib}(\Xbstar)\cdot \left(1-\Q_{\Xiaib}(\Xbstar)\right)} \right)\,,
\end{align}
for some probability measure $\Q$ on \X. We additionally included the square root of the second criterion from \eqref{eq:Rob_Loc_Versch_DiffRegPartII} since it will arise in the proof of the subsequent \Cref{Thm:Rob_Loc_VerschAuftLp} that this square root is also relevant to the difference we want to investigate.

Finally, we also need to introduce some new notation because of the already mentioned auxiliary SVMs on the sets $\Xbstar[1],\dots,\Xbstar[B]$ from \textbf{(R2')} which we will need for proving our stability results: We will denote the auxiliary distributions, regularization parameters and kernels we need for this by using the $(\cdot)^*$-notation. That is, $\Pibstar:=\P_{i,\Xbstar}$, $\lbijbstar:=(\Pjaibx{j}(\Xbstar))^{-1}\lbiaib$ and  $\kibstar:=\kiaib\einschraenkung_{\Xbstar\times\Xbstar}$, $i,j=1,2$, $b=1,\dots,B$. Here, \aib denotes that index $a\in\{1,\dots,A_i\}$ such that $\Xbstar\subseteq\Xia$, which is well-defined because of \textbf{(R2')} (existence of such an index) and \textbf{(R1')} (uniqueness of that index). Lastly, because of Lemma 4.3 from \cite{steinwart2008}, \kibstar is actually an kernel again.

With this, we can now state our stability result. As seen before, we will not be able to derive meaningful results regarding the uniform norm of the difference of two localized SVMs based on different regionalizations. However, it is indeed possible to obtain a meaningful bound on the \Lapix-norm of this difference:

\begin{mythm}\label{Thm:Rob_Loc_VerschAuftLp}
	Let \X be a complete and separable metric space and $\Y\subseteq\R$ be closed. Let $\P_1,\P_2\in\MXY$ be probability measures. Let $\XiAibold:=\{\X_{i,1},\dots,\X_{i,A_i}\}$, $i=1,2$, be regionalizations of \X such that \XiAibold[1] and \XiAibold[2] both satisfy \textbf{(R1')} and that they together satisfy, for $\P_1$ as well as for $\P_2$, \textbf{(R2')}. Let $\lbia>0$ and let $\kia$ be a bounded and measurable kernel with separable RKHS $\Hia$ for all $i\in\{1,2\}$ and $a\in\{1,\dots,A_i\}$. Denote $\kappa_b:=\max\{\normSup{\kiaib[1]},\normSup{\kiaib[2]}\}$, $\tau_b:=\min\{\lbiaib[1],\lbiaib[2]\}$ and $\rho_{1,b}:=\max\left\{\Pix[1](\Xiaib[1]),\Pix[1](\Xiaib[2])\right\}$ for all $b\in\{1,\dots,B\}$. Let \loss be a convex and Lipschitz continuous loss function. Let \fiextreg[1] and \fiextreg[2] be defined as in \eqref{eq:Rob_Loc_DefGlobalPredictor} with the weight functions $w_1,\dots,w_B$ satisfying \textbf{(W1)}, \textbf{(W2)} and \textbf{(W3)}. Then, \red{Natürlich auch vertauschen von 1 und 2 möglich. Irgendwie anmerken, da es bei anderen Resultaten mit $\P_i$ statt $\P_1$ gemacht wurde?}
	\begin{align*}
		&\normLapix[1]{\fiextreg[1]-\fiextreg[2]}\\
		&\le |\loss|_1 \cdot \sum_{a=1}^{A_{2}} \Pix[1](\Xia[2]) \cdot \frac{\normSup{\kia[2]}^2}{\lbia[2]} \cdot \norm{tv}{\Pjai[2]{1}-\Pjai[2]{2}}\\
		&\hspace*{0.4cm} + |\loss|_1 \cdot \sum_{b=1}^B \bigg( \rho_{1,b}\cdot\frac{\kappa_b^2}{\tau_b^2} \cdot \left|\lbiaib[1] - \lbiaib[2] \right|\\
		&\hspace*{2.5cm} + \Pix[1](\Xbstar) \cdot \left(\frac{1}{2\tau_b} \cdot \normLapibstarxb[1]{\kibstar[1,b]-\kibstar[2,b]} + \frac{\kappa_b}{\tau_b} \cdot \sqrt{\normLapibstarxb[1]{\kibstar[1,b]-\kibstar[2,b]}} \right)\\
		&\hspace*{2.5cm} + \rho_{1,b} \cdot \frac{\kappa_b^2}{\tau_b} \cdot \distReg{\P_1}(\XiAibold[1],\XiAibold[2]) \bigg)\,.
	\end{align*}
	\red{Teil mit tv-Norm kann auch als Summe über B dargestellt werden (über a(2,b)). Ist an sich unnötig, würde Summen aber vereinheitlichen. Außerdem: Hier nur L1-Norm, vorher immer allgemeine Lp-Norm. Erklären, weshalb!}
\end{mythm}

